Towards Better Agents for Multi-Turn User Interaction: The Next User Turn Is More Than Context

User-facing tool agents must coordinate dialogue and tool use as user goals unfold over multiple turns. Yet interactive reinforcement learning typically reduces each rollout to a terminal reward, assigning the same credit to effective elicitation, errors, and later repair. The next user turn is more than context: it also provides noisy, temporally local evidence about the preceding user-to-user segment. We introduce \textbf{F}eedback-\textbf{A}ware \textbf{C}redit \textbf{A}ssignment (\textsc{FACA}), which aligns each reaction with that segment, derives a locally normalized reaction advantage, and adds it to verified terminal outcome advantage without an extra critic or rollout. Against an outcome-only Interactive GRPO control matched in simulator, visible dialogue, initialization, rollout, and optimization, \textsc{FACA} improves the nine-domain $\tau$-family average across three independently trained runs by 5.91 and 10.22 percentage points at 8B and 14B, respectively. Gains concentrate in Telecom; at 8B, randomizing reaction polarity removes the Telecom gain. The same ordering holds zero-shot on Pare-Bench and Co-Gym. These results demonstrate that next-turn user reactions provide actionable local credit for improving multi-turn user-interacting agents.

==> sections/00_abstract.tex <==
\begin{abstract}
User-facing tool agents must coordinate dialogue and tool use as user goals
unfold over multiple turns. Yet interactive reinforcement learning typically
reduces each rollout to a terminal reward, assigning the same credit to
effective elicitation, errors, and later repair. The next user turn is more
than context: it also provides noisy, temporally local evidence about the
preceding user-to-user segment. We introduce \textbf{F}eedback-\textbf{A}ware \textbf{C}redit
\textbf{A}ssignment (\FACA{}), which aligns each reaction with that segment,
derives a locally normalized reaction advantage, and adds it to verified
terminal outcome advantage without an extra critic or rollout. Against an
outcome-only Interactive GRPO control matched in simulator, visible dialogue,
initialization, rollout, and optimization, \FACA{} improves the nine-domain
$\tau$-family average across three independently trained runs by 5.91 and 10.22
percentage points at 8B and 14B, respectively. Gains concentrate in Telecom;
at 8B, randomizing reaction polarity removes the Telecom gain. The same
ordering holds zero-shot on Pare-Bench and Co-Gym. These results demonstrate that next-turn user reactions provide actionable local credit for improving multi-turn user-interacting agents.
\end{abstract}


==> sections/10_ethics.tex <==
\section*{Ethical Considerations}

This work trains agents against simulated users and does not introduce a human
participant study in its current form. Nevertheless, optimizing coarse user-
reaction labels can encourage agreement-seeking, manipulation, unnecessary dialogue,
or violations of domain policy. We therefore treat task correctness and policy
compliance as primary constraints and reaction evidence only as auxiliary credit.
Any deployment with real users would require consent, privacy protection,
domain-specific safety checks, and monitoring for disparate behavior across
user groups. Simulator-generated trajectories may also encode biases from the
underlying model and should not be interpreted as representative human
preferences.


==> tables/related_work.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{0.14\textwidth}
                >{\raggedright\arraybackslash}p{0.20\textwidth}
                >{\raggedright\arraybackslash}p{0.27\textwidth}
                >{\raggedright\arraybackslash}p{0.29\textwidth}@{}}
\toprule
\textbf{Signal source} & \textbf{Representative methods} & \textbf{Local signal} & \textbf{Distinction from FACA} \\
\midrule
Terminal outcome & GRPO, MUA-RL, UserRL & One trajectory score, broadcast or redistributed & Reactions remain observations rather than explicit local credit \\
Learned evaluator / value & PRM800K, Math-Shepherd, AgentPRM, ArCHer, SWEET-RL, Agent Lightning & Process label, value estimate, verifier, or credit module & Requires a learned or task-specific intermediate estimator \\
Implicit user feedback & Follow-up likelihood, RLUF & Follow-up likelihood or predicted production reaction & Optimizes response preference or satisfaction through a learned reward model \\
Policy belief / information & IGPO, InfoPO, SIOP & Belief change, counterfactual information gain, or latent outcome potential & Requires answer semantics, extra policy evaluations, or outcome clustering \\
Rollout-derived decomposition & SPO, AT$^2$PO, GiGPO & Monte Carlo segment return, tree propagation, or repeated-anchor comparison & Requires additional continuations, branches, or recurring states \\
Structured / intrinsic process cues & RLVMR, TEPO & Verifiable meta-reasoning event or entropy change around a tool call & Uses tagged cognition or model uncertainty rather than partner feedback \\
Homogeneous-group repair & AVSPO & Adaptive virtual reward samples & Restores relative variation without using partner behavior \\
Simulator state & EIBench / CTC-GRPO & Change in privileged emotion--relation state & Uses a scalar latent simulator state \\
\textbf{User reaction} & \textbf{FACA} & \textbf{Next-user confirmation, correction, confusion, rejection, or neutral event} & \textbf{Same-rollout partner behavior; observable extraction remains to be validated} \\
\bottomrule
\end{tabular*}
\caption{Turn-level credit methods differ most clearly by the source of their
local signal. FACA's novelty claim concerns reaction events, not the general
existence of turn-level or two-level advantages.}
\label{tab:related-work}
\end{table*}

